Data-driven optimal control under safety constraints using sparse Koopman approximation

In this work we approach the dual optimal reach-safe control problem using sparse approximations of Koopman operator. Matrix approximation of Koopman operator needs to solve a least-squares (LS) problem in the lifted function space, which is computationally intractable for fine discretizations and high dimensions. The state transitional physical meaning of the Koopman operator leads to a sparse LS problem in this space. Leveraging this sparsity, we propose an efficient method to solve the sparse LS problem where we reduce the problem dimension dramatically by formulating the problem using only the non-zero elements in the approximation matrix with known sparsity pattern. The obtained matrix approximation of the operators is then used in a dual optimal reach-safe problem formulation where a linear program with sparse linear constraints naturally appears. We validate our proposed method on various dynamical systems and show that the computation time for operator approximation is greatly reduced with high precision in the solutions.

==> LP_formulation.tex <==
\section{Sparse Convex optimal control formulation}
\label{sec:LP_SDP}
{\chen combine section V, VI.} After solving the sparse least-squares problem (\ref{eq:sp_normeq_lin}) for $\bv$ and using operator $\mathscr{K}^+$ mapping $\bv$ to the sparse $\bK$, we obtained a sparse representation of the Koopman and P-F operator. In this section we leverage the sparsity of the matrix $\bK$ and $\bP$, formulating the optimal control problem under safety constraints (\ref{eq:eq_main}) into a linear program with sparse constraints.
\subsection{L1 input-regularized problem and linear programming}
 We show that problem (\ref{eq:eq_main}) naturally leads to a linear programming in the lifted space defined by the linear span of $\bPsi$. By the definition of P-F infinitesimal generator (\ref{eq:PF_generator}), the equality constraint 
 \begin{equation}
     {\color{red} \nabla\cdot [({\mathbf{f} + \bg \bu})\rho](\bx) = -[{\cal{P}}_{\mathbf{f}+\bg\bu}]\rho(\bx) \approx \bv^T (\frac{\bI-\bP}{\Delta t}  \bPsi).  }
     \label{eq:PF_approx}
 \end{equation}

and it is straightforward to show that problem (\ref{eq:LP_convex}) can be further formulated as LP.
\begin{equation}
\begin{split}
\inf_{\bv, \bw_1,\dots,\bw_m, \bs_1,\dots,\bs_m} &\;\;\bI_q^T\bv + \sum_{i=1}^m\bI_{\Psi}^T\bs_i \\ 
    \textrm{s.t.} &\;\;\;\; {\color{red}\sum_{i=0}^m} \frac{\bI - \bP_i}{\Delta t}\bw_i = \bh\\
    &\;\;\;\; \bI_{\bX_u}^T\bv = 0\\
    &\;\;\;\; \bs_i \geq \lvert \bw_i \rvert, i=1, \dots, m\\
    &\;\;\;\; \lvert \bw_i \rvert \leq u_{max} \bv, i=1, \dots, m
\end{split}
\label{LP}
\end{equation}
where 
\begin{equation}
    \begin{split}
        &\bI_q = \int_{\bX} q(\bx)\bPsi(\bx) d\bx, \;\;\; \bI_{\bPsi} = \int_{\bX} \bPsi(\bx) d\bx,\\
        &\bI_{\bX_u} = \int_{\bX} \indicator_{\bX_u} \bPsi(\bx) d\bx
    \end{split}
\end{equation}
are constants and can be integrated before-hand, and $\bs_i, i=1,\dots,m$ are slack variable coefficients, and $\bP_i, i=1,\dots, m$ are sparse representations for P-F infinitesimal generators (\ref{eq:PF_generator}) obtained in section \ref{sec:sparse_approx}. Notice that in formulation (\ref{LP}) we added additional constraints $\lvert \bw_i \rvert \leq \alpha \bv, i=1, \dots, m$. This is an indirect enforcement of the bounded control input constraint
\begin{equation}
    \lvert \bu \rvert \leq u_{max}.
\end{equation}
The bounded input constraint corresponds to the modeling of actuation limits in the real-world machines and autonomous systems. It is worth mentioning that this constraint also guarantees our LP formulation (\ref{LP}) to have a meaningful solution, as if without this constraint the minimum value is always zero by choosing $\bv=\mathbf{0}, \bw_i=\mathbf{0}, i=1,\dots,m$.

